Colmena: Scalable Machine-Learning-Based Steering of Ensemble Simulations for High Performance Computing

Scientific applications that involve simulation ensembles can be accelerated greatly by using experiment design methods to select the best simulations to perform. Methods that use machine learning (ML) to create proxy models of simulations show particular promise for guiding ensembles but are challenging to deploy because of the need to coordinate dynamic mixes of simulation and learning tasks. We present Colmena, an open-source Python framework that allows users to steer campaigns by providing just the implementations of individual tasks plus the logic used to choose which tasks to execute when. Colmena handles task dispatch, results collation, ML model invocation, and ML model (re)training, using Parsl to execute tasks on HPC systems. We describe the design of Colmena and illustrate its capabilities by applying it to electrolyte design, where it both scales to 65536 CPUs and accelerates the discovery rate for high-performance molecules by a factor of 100 over unguided searches.

==> ccs.tex <==
%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
\begin{CCSXML}
<ccs2012>
 <concept>
  <concept_id>10010520.10010553.10010562</concept_id>
  <concept_desc>Computer systems organization~Embedded systems</concept_desc>
  <concept_significance>500</concept_significance>
 </concept>
 <concept>
  <concept_id>10010520.10010575.10010755</concept_id>
  <concept_desc>Computer systems organization~Redundancy</concept_desc>
  <concept_significance>300</concept_significance>
 </concept>
 <concept>
  <concept_id>10010520.10010553.10010554</concept_id>
  <concept_desc>Computer systems organization~Robotics</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
 <concept>
  <concept_id>10003033.10003083.10003095</concept_id>
  <concept_desc>Networks~Network reliability</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computer systems organization~Embedded systems}
\ccsdesc[300]{Computer systems organization~Redundancy}
\ccsdesc{Computer systems organization~Robotics}
\ccsdesc[100]{Networks~Network reliability}

==> taxonomy.tex <==
\subsection{Comparison to Other Steering Frameworks}\label{sec:programming-model}
\logan{Should this go before or after we describe our approach? I think ``after'' so we introduce features before comparing them to existing platforms}
\ryan{I think this is good here. I wonder about 3.3's placement though? Maybe it isn't necessary? or could move to eval}

Colmena is modeled after existing tools for steering ensemble simulations with the goal of providing a more flexible route for specifying steering policies.
At a basic level, Colmena shares the separation of software into ``task generation'' and ``task execution'' components common across most steering software.
The differences between the task execution components are important, but somewhat irrelevant given Colmena and other steering frameworks (e.g., libEnsemble\cite{libEnsemble},
DeepHyper\cite{balaprakash2018deephyper}) can use different workflow engines for asynchronous task execution.
Flexibility is important given the range in needs for scientific application, such as Swift/T supporting high execution rates of short-duration tasks and Fireworks/Balsam providing persistent tracking of longer-duration tasks.\logan{@Kyle: Sound fair? Could I cite your ExaWorks paper for further discussion}
Consequently, we ensured Colmena was not tied to a specific execution toolkit and invested more time in deciding hwo to express planning policies.

Many different models for expressing steering algorithms are evident in the literature.
We drew inspiration from these different approaches when creating the architecture and programming model for Colmena.
Here, we outline the various models, how we used them to design Colmena and what new capabilities Colmena provides:
\begin{itemize}
    \item \textit{Main Loop}: \logan{``Centralized''} A persistent main function updates a task list by submitting new tasks and reading results from a task queue.
    \begin{itemize}
        \item Advantages: Strong separation between planning and execution allows easily switching workflow engines, planning logic is consolidated to a single process
        \item Examples: CANDLE Supervisor,\cite{wozniak2018supervisor} DeepHyper.\cite{balaprakash2018deephyper}
        \item Influence: Colmena communicates to a task server via a queue, control is degrated to a central process
        \item Improvement: Colmena simplifies writing multiple, cooperative planning threads to facilitate writing complex policies.
    \end{itemize}
    
    \item \textit{Producer/Consumer}: The application is split into ``consumer'' tasks that perform assays based on points suggested by ``producer'' tasks based on previous assays.
    A central manager maintains the assay history and the number of workers running each type of task
    \begin{itemize}
        \item Advantages: Increasing the rate of decision making can be achieved by scaling the number of producer tasks.
        \item Examples: libEnsemble\cite{libEnsemble}
        \item Influence: Colmena can run multiple planning tasks (e.g., model training, inference) concurrently to achieve strong scaling rates
        \item Difference: Colmena enables writing policies that are hard to express a pair of consumer/producer functions, such as by introducing a third agent to prioritize samples generated by multiple producer functions.
    \end{itemize}
    
    \item \textit{Workflow-Based}: \logan{``Decentralized''} Planning tasks expressed as a step in a workflow graph that is capable of adding new steps to the graph.\logan{@Kyle: Are ``steps'' and ``graphs'' good terms/well-understood concepts?}
    \begin{itemize}
        \item Advantages: Workflows are natural forms for expressing complex relationships between assay and planning tasks or events which trigger planning.
        \item Examples: Rocketsled\cite{dunn2019rocketsled}
        \item Influence: Colmena provides simple routes for triggering actions after workflow steps complete.
        \item Difference: Colmena can easily be ported to different execution engines
    \end{itemize}
    
    \item \textit{Actor-based}: The planning task is broken into multiple interacting agents that can each run on different computers. Once deployed, agents communicate information (e.g., assay results, new tasks) via pre-defined routes.
    \begin{itemize}
        \item Advantages: Logic for responding to certain kinds of events separated into discrete agents, planning agents may perform tasks asynchronously
        \item Examples: Ray\cite{mortiz2018ray}
        \item Influence: Colmena policies are written as multiple interacting threads
        \item Difference: Colmena tasks are executed on stateless workers, simplifying multi-site deployments.
    \end{itemize}
\end{itemize}

In short, Colmena provides a toolkit that was purpose-built for expressing the complex policies needed to efficiently use highly-parallel supercomputers for computational campaigns.

